All Nodes are created Not Equal: Node-Specific Layer Aggregation and Filtration for GNN

The ever-designed Graph Neural Networks, though opening a promising path for the modeling of the graph-structure data, unfortunately introduce two daunting obstacles to their deployment on devices. (I) Most of existing GNNs are shallow, due mostly to the over-smoothing and gradient-vanish problem as they go deeper as convolutional architectures. (II) The vast majority of GNNs adhere to the homophily assumption, where the central node and its adjacent nodes share the same label. This assumption often poses challenges for many GNNs working with heterophilic graphs. Addressing the aforementioned issue has become a looming challenge in enhancing the robustness and scalability of GNN applications. In this paper, we take a comprehensive and systematic approach to overcoming the two aforementioned challenges for the first time. We propose a Node-Specific Layer Aggregation and Filtration architecture, termed NoSAF, a framework capable of filtering and processing information from each individual nodes. NoSAF introduces the concept of "All Nodes are Created Not Equal" into every layer of deep networks, aiming to provide a reliable information filter for each layer's nodes to sieve out information beneficial for the subsequent layer. By incorporating a dynamically updated codebank, NoSAF dynamically optimizes the optimal information outputted downwards at each layer. This effectively overcomes heterophilic issues and aids in deepening the network. To compensate for the information loss caused by the continuous filtering in NoSAF, we also propose NoSAF-D (Deep), which incorporates a compensation mechanism that replenishes information in every layer of the model, allowing NoSAF to perform meaningful computations even in very deep layers.

==> chapters/current_reg.tex <==



\section{Regularization in Current Explainability} \label{part:p}
To ensure the size and quality of the explanatory subgraphs, most existing mask-based explanation methods adopt regularization terms to enhance the explanation generations. Specifically, these regularization terms are introduced to constrain the values of the mask. In general, we categorize these regularization terms into two types. The first type pertains to regularizations that constrain the size of the subgraphs. These regularizations primarily involve constraining the amount of information contained within the subgraphs. They act directly upon the values of the constraint mask and include those based on magnitude, budget, and information bottleneck (IB). Figure \ref{fig:reg} roughly illustrates the relationship between the intensity of the constraints (vertical axis) applied by these three methods and the value of the mask (horizontal axis). Specifically,
\begin{itemize}
    \item  As shown in  Figure \ref{fig:reg} (a), the size of the \textbf{magnitude-based} regularization term is directly proportional to the magnitude of the mask, constraining the overall mask values within a narrow range \cite{GNNEx,CF-GNNEx,Refine};
    \item The \textbf{budget-based} regularization term is zero when the mask's value is within a certain range, implying no constraint is applied, as exhibited in  Figure \ref{fig:reg} (b). However, once this threshold is exceeded, its effect is similar to that of the magnitude-based regularization, with the upper limit of this range being the "budget" \cite{PGEx,GraphMASK,AIA,GREA}; 
    \item The \textbf{IB-based} regularization term as illustrated in Figure \ref{fig:reg} (c) attempts to bind the mask's value to a predetermined target, with the regularization magnitude proportional to the distance from the mask's value to this preset target \cite{GSAT}.
\end{itemize}
The second type involves constraints on the structure of the subgraphs. These regularizations mainly include constraining the internal connectivity of the subgraphs and the discreteness of the mask values:
\begin{itemize}
    \item  \textbf{Connectivity constraints} tend to bring edges or nodes with larger mask values closer to each other \cite{PGEx,GIB_sub}. In such cases, when edges are selected to form an explanatory subgraph based on the size of the mask, the resulting subgraph is likely to be tightly connected, reducing the occurrence of isolated points within the explanatory subgraphs; 
    \item \textbf{Discreteness constraints}, on the other hand, strive to push the mask values away from 0.5 and towards 0 or 1, thus minimizing the difference between the amount of information carried by the selected edges or nodes and the information they carried during the training process \cite{GNNEx,PGEx,AIA,GREA}.
\end{itemize}

\noindent Table \ref{table:intro} presents the categories of regularization terms applied by the current mainstream mask-based post-hoc and intrinsic graph interpretability algorithms, where we have also collated the target norms of the regularization terms used by each interpretability method, namely, the $\ell_0$, $\ell_1$, or $\ell_2$ norms.




==> chapters/related.tex <==
\begin{table}[htp]
% \vspace{-5pt}
\caption{The performance of baseline explainers averaged across 10 runs. The best performing methods are bold, and the strongest baselines are underlined.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\toprule
                & BA3-motif         & Mutagenicity      & MNIST             \\
\midrule\midrule
GNNExplainer    & 0.439\std{0.024}  & 0.841\std{0.022}  & 0.798\std{0.047}  \\
{\quad+ORS}     & 0.466\std{0.033}  & 0.860\std{0.031}  & 0.814\std{0.054}  \\
\midrule
PGExplainer     & 0.511\std{0.032}  & 0.809\std{0.055}  & 0.800\std{0.050}  \\
{\quad+ORS}     & 0.537\std{0.019}  & 0.821\std{0.026}  & 0.813\std{0.027}  \\
\midrule
GraphMask       & 0.489\std{0.051}  & 0.826\std{0.056}  & 0.817\std{0.047}  \\
{\quad+ORS}     & 0.496\std{0.042}  & 0.844\std{0.011}  & 0.828\std{0.053}  \\
\midrule
CF-GNNExplainer & 0.453\std{0.044}  & 0.842\std{0.038}  & 0.822\std{0.037}  \\
{\quad+ORS}     & 0.470\std{0.046}  & 0.853\std{0.029}  & 0.844\std{0.025}  \\
\midrule
Refine          & 0.542\std{0.031}  & \underline{0.905}\std{0.055}  
                                                        & 0.854\std{0.062}  \\
{\quad+ORS}     & 0.551\std{0.017}  & \textbf{0.911}\std{0.018}         
                                                        & 0.866\std{0.030}  \\
\midrule
GSAT            & \underline{0.582}\std{0.027} 
                                    & 0.892\std{0.031}  & \underline{0.871}\std{0.042}
                                                                            \\ 
{\quad+ORS}     & \textbf{0.591}\std{0.023} 
                                    & 0.903\std{0.035}  & \textbf{0.883}\std{0.017}
                                                                            \\
\midrule
\textbf{Relative Impro.}  
                & \textbf{3.3$\%$}  & \textbf{3.6$\%$}  & \textbf{3.1$\%$}  \\
\bottomrule
\end{tabular}}
\label{tab:exp_ors}
% \vspace{-10pt}
\end{table}
% -----------------------------------------------------------------------------


\section{Related Work} \label{part:related}

In this section, we briefly introduce the explanation methods tailored for GNNs \cite{SAEx, CAM, SubgraphX, Gem}, especially the  mask-based methods \cite{GREA,GIL,GIB,GIB_sub}. GNNExplainer \cite{GNNEx} directly learns an adjacency matrix mask through maximizing the mutual information between a GNN’s prediction and distribution of possible subgraph structures, which is performed via multiplying the mask to the input features. PGExplainer \cite{PGEx} adopts a deep neural network to parameterize the generation process of explanations, which makes it a natural approach to explaining multiple instances collectively.  It can also provide global explanations for a certain class.
GraphMask \cite{GraphMASK} learns a simple classifier that, for every edge in every layer, predicts if that edge can be dropped, in a fully differentiable fashion. Then by dropping edges without deteriorating the performance of the model, the remaining edges naturally form an explanation for the model's prediction.
CF-GNNExplainer \cite{CF-GNNEx} focuses on the counterfactual explanations by figuring out the minimal perturbation to the input graph such that the prediction changes. By instantiating the perturbation with only edge deletions, they find out the edges which are crucial.
Refine \cite{Refine} develops an explainer that can generate multi-grained explanations by exploiting the pre-training and fine-tuning idea. Specifically, the pre-training phase exhibits global explanations with the prototypical patterns, and the fine-tuning phase further adapts the global explanations in the local context with high fidelity.
GSAT \cite{GSAT} leverages stochastic attention to block the information from the task-irrelevant graph components while learning stochasticity-reduced attention to select the task-relevant subgraphs for interpretation. Though it's naturally an inherently interpretable method, it also works in a post-hoc way through a fine-tuning fashion. We adopt this post-hoc working mode as one baseline.


% \textbf{Feature attribution.} Current explainers mainly perform feature attribution by leveraging:
% \begin{itemize}[leftmargin=*,topsep=0pt]
%     \setlength{\itemsep}{0pt}
%     \setlength{\parsep}{0pt}
%     \setlength{\parskip}{0pt}
%     \item Gradient-like signals \textit{w.r.t.} the graph structure \cite{SAEx, CAM}. For example, SA \cite{SAEx} directly calculates the  gradients of GNN’s loss \textit{w.r.t.} adjacency matrix as the importance scores;
%     \item Attention scores of structural features \cite{PGEx, GSAT}. For example, GSAT (in its post-hoc working mode) \cite{GSAT} trains a parameterized predictor to generate the  attention score for each edge as their importance via the stochastic mechanism;
%     \item Mask scores of structural features \cite{GNNEx, Refine}. For example, GNNExplainer \cite{GNNEx} adds soft masks to the input features and trains them by maximizing the mutual information between the masked outcome and target prediction;
%     \item  Prediction changes on structure perturbations \cite{SAEx, CAM, SubgraphX, Gem}. For example, PGMExplainer \cite{PGMEx} collects the prediction change on the random node perturbations and learns a Bayesian network from these observations.
% \end{itemize}

% \noindent \textbf{Feature selection.} With attribution scores of features, input features are sequentially filled into the set of salient features to generate the explanatory subgraph according to their importance rank. Many regularization terms are introduced to guide this process. For example, sparsity constraints \cite{GNNEx, GraphMASK} typically leverage the $l_1$ norm to guarantee that the selected subgraph remains within a prescribed size; connective constraints \cite{PGEx, Refine} give more selective probabilities to the edges connecting with the part selected already; more recently, information bottleneck constraints \cite{GSAT, wang2022searching} are proposed to squeeze the mutual information between the input graph and the selected subgraph. More recently, CGE aims to leverage the lottery ticket hypothesis to prune and explain the GNN \cite{wang2022searching,wangkun2023snowflake} rather than explain input graphs. 

==> chapters/rethink.tex <==
\section{Rethinking the Role of Regularization} \label{part:Rethink}

\begin{figure*}[htp]
\setlength{\abovecaptionskip}{6pt}
\centering
\includegraphics[width=0.9\textwidth]{figures/icml11.png} 
\caption{The role of regularization in the phases of feature attribution and feature selection.}
\label{fig:two_phases}
\end{figure*}


In this section, we critically evaluate the function of regularization within the context of GNN explainers, informed by the GIBE framework established previously. We dissect the influence of regularization across two critical stages of the explanation process: feature attribution and feature selection in Section \ref{part:Two Phase}. This bifurcation allows for a precise understanding of how regularization impacts each phase distinctly.

Subsequent to this analysis, we derive three compelling propositions under the guidance of GIBE. These propositions elucidate the connections between regularization and three pivotal elements in the domain of GNNs explainability: sparsity, stochastic mechanisms, and the out-of-distribution (OOD) issue, as referenced in the literature \cite{GNNEx,CF-GNNEx,PGEx,Refine,GSAT,DIR}. Each proposition offers an insight into how regularization interacts with these aspects to shape the quality and reliability of explanations provided by GNNs.

Inspired by the theoretical insights gleaned from these propositions, we introduce two novel regularization schemes. These schemes are designed to be both straightforward and potent, aimed at augmenting the efficacy of extant explanation methodologies. By incorporating these schemes, we aim to not only enhance the interpretative power of GNNs but also to address some of the persistent challenges in the field such as balancing sparsity with explanatory depth.


\subsection{Regularization in Two Phases} \label{part:Two Phase}
% Regularization is widely recognized by its extraordinary power to prevent the overfitting and endowing the generalization \cite{regular_1,regular_2}. Since interpreting an input graph appeals no ability of generalization, we leverage GIBE to rethink the role of regularization  from the perspective of information theory.
% As the preparation, GIBE  combines the principle of GIB and the common paradigm of the explanation methods (\textit{i.e.}, feature attribution and selection). Specifically, the first term of Equation \ref{eq:GEIB} is the optimization objective of feature attribution, which maps the information of feature importance in $\mathcal{G}$ to mask, $\mathcal{G}\mapsto\mathcal{G}\odot\mathbf{M}$; and the second term is the objective of feature selection,  which maps the information in the mask to subgraph to get the optimal subgraph $\mathcal{G}^\ast$, $\mathcal{G}\odot\mathbf{M}\mapsto\mathcal{G}_s$. In conclusion, GIBE endows the GIB with better ability to directly guide the construction of the explanation methods.

\textbf{Regularization in feature attribution.} 
% To perform the mapping $\mathcal{G} \mapsto \mathcal{G}\odot \mathbf{M}$ in feature attribution, considering the latent distribution $\Space{P}(\mathcal{G}_s,\mathbf{Y})$ is intractable, existing  methods inevitably treating $f(\cdot \,|\, \Theta)$ as the proxy function to estimate the $ I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right)$ according to:
Directly calculating the training objective of feature attribution, $ I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right)$ is tough since the latent distribution $\Space{P}(\mathcal{G} \odot \mathbf{M} ,\mathbf{Y})$ is notoriously intractable. Hence, existing explainers typically introduce the parameterized variational approximation $\mathbb{P}_\theta\left(\mathbf{Y}\,|\,\mathcal{G} \odot \mathbf{M} \right)$ for $\mathbb{P}\left(\mathbf{Y}\,|\,\mathcal{G} \odot \mathbf{M} \right)$ according to:
\begin{equation} \label{eq:OOD_attri_all}
\begin{aligned}
& I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right) = \mathbb{E}_{\mathcal{G} \odot \mathbf{M}, \mathbf{Y}}\left[\log \mathbb{P}_\theta\left(\mathbf{Y}\,|\,\mathcal{G} \odot \mathbf{M} \right)\right]+H(\mathbf{Y}) \\
&+\mathbb{E}_{\mathcal{G} \odot \mathbf{M} }\left[\operatorname{KL}\left(\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right) ||\, \mathbb{P}_\theta\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right)\right)\right],
\end{aligned}
\end{equation}
where $\operatorname{KL}(\cdot||\cdot)$ is the Kullback-Leibler divergence.

Detailed derivation is provided in Appendix. Treating classifier $f$ as the proxy function of $\Space{P}_\theta$, the first term of Equation \ref{eq:OOD_attri_all} can be specified as the cross-entropy between $\mathbf{Y}$ and $f(\mathcal{G} \odot \mathbf{M} )$. In this case, since the second term $H(\mathbf{Y})$ is a constant, the gap between $I\left(\mathcal{G} \odot \mathbf{M}; \mathbf{Y}\right)$ and the above cross-entropy, shown as \textit{gap1} in Figure \ref{fig:two_phases}, solely depends on the third term of Equation \ref{eq:OOD_attri_all}. Note that this term is also the Kullback-Leibler (KL) Divergence \cite{KL} between $\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)$ and $f(\mathcal{G} \odot \mathbf{M})$. 
%未标注KL  注意！

% the Kullback-Leibler (KL) Divergence between $\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)$ and $\mathbb{P}_\theta\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)$

% where $\mathbb{E}_{\mathcal{G} \odot \mathbf{M}, \mathbf{Y}}\left[\log \mathbb{P}_{\theta}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)\right]$ is always specified as the cross-entropy between $\mathbf{Y}$ and $f(\mathcal{G} \odot \mathbf{M} \,|\, \Theta)$ using above proxy function. Since the second term $H(\mathbf{Y})$ is a constant, the gap between $I\left(\mathcal{G} \odot \mathbf{M}; \mathbf{Y}\right)$ and above cross-entropy solely depends on the third term: the Kullback-Leibler (KL) Divergence between $\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)$ and $\mathbb{P}_\theta\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)$. 

To bridge this gap and maximize the effectiveness of feature attribution,  regularization should play a role in constraining $\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right)$ to $f$. Since $f$ is trained for data distribution ${P}(\mathcal{G},\mathbf{Y})$, this role is transferred to constrain $\mathcal{G}\odot \mathbf{M}$ to $\mathcal{G}$. In this case, the constraint orientation of $\mathbf{M}$ should be loosened to $\mathbf{A}$ to squeeze gap in feature attribution to 0, as shown in the left side of Figure \ref{fig:two_phases}.

\textbf{Regularization in feature selection.} Feature selection typically binarizes $\mathbf{M}$ to achieve the mapping $\mathcal{G}\odot \mathbf{M} \mapsto \mathcal{G}^\ast$. To bridge the gap between $\mathbf{M}$ and its binaryzation $\mathbf{M'}$, shown as \textit{gap2} in Figure \ref{fig:two_phases}, the optimization objective of feature selection, $-I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}\right)+I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}^\ast\right)$ in Equation \ref{eq:GEIB} is usually maximized by various regularization terms, such as Budget- and IB-based constraints. In Figure \ref{fig:reg2}, we elucidate the approximate relationship between prevalent regularization strategies and the objective function during the feature selection phase. The figure's left panel graphically represents the trends of the two terms within the objective function. We postulate that explainability algorithms tacitly evaluate the significance of these terms in response to the empirical conditions. As depicted in the right panel of Figure  \ref{fig:reg2}, a predominance of the first term (\textit{i.e.}, $I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}\right)$) suggests an inclination towards magnitude-based regularization methods. Conversely, a greater weight on the second term (\textit{i.e.}, $I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}^\ast\right)$) indicates a preference for IB methods. In scenarios where both terms are of comparable importance, budget-based regularization methods are likely to emerge as the summative approach.

In summary, in the phase of feature selection, regularization plays a role in constraining $\mathcal{G}\odot \mathbf{M}$ to $\mathcal{G}^\ast$. In other words, the constraint orientation of $\mathbf{M}$ should be tightened to $\mathbf{A}_s$ (\textit{i.e.}, adjacency matrix of $\mathcal{G}^\ast$) for squeezing the gap in feature selection to 0, as shown in the right side of Figure \ref{fig:two_phases}.


% To achieve the mapping $\mathcal{G}\odot \mathbf{M} \mapsto \mathcal{G}_s$ in feature selection, existing explainers typically binarize $\mathbf{M}$ to maximize $I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}^\ast\right)-I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}\right)$. To bridge the gap between $\mathbf{M}$ and its binaryzation $\Mat{M'}$, typically, (1) discrete constraint \cite{GNNEx} works for maximizing the first term: $I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}^\ast\right)$; (2) sparsity constraint leverages the $l_1$ or $l_2$ norm to minimize the second term:

% To this end,  $I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}\right)$. In this case, regularization should play a role in constraining $\mathcal{G}\odot \mathbf{M}$ to $\mathcal{G}^\ast$ to bridge the gap between $\mathbf{M}$ and its binaryzation.

\textbf{Role of Regularization.} In conclusion,  while the constraint orientation of $\mathbf{M}$ is beneficial to feature attribution and the gap in feature attribution tends to zero, the gap in feature selection will inevitably become large, and vice versa. In other words, since the role of regularization is totally different across two phases, regularization  is essentially a tradeoff to guarantee the mapping effectiveness both in two phases:

\textit{\textbf{Proposition 4.1 (Role of Regularization)}
Regularization in GNNs explainability is essentially the tradeoff scheme to pursue the balance between the phases of feature attribution and feature selection.}


% \section{Propositions of Regularization in Explanation methods } \label{part:Novel}

% In this section, we derive three intriguing propositions stemming from GIBE and Proposition \ref{prop:essence}, which respectively reveal the relation between regularization and three important concepts in GNNs explainability (\textit{i.e.}, sparsity \cite{GNNEx,CF-GNNEx}, stochastic mechanism \cite{PGEx,Refine} and OOD issue \cite{GSAT,DIR}). Inspired by these propositions, we propose two simple yet effective   regularization schemes.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Sparsity \& Regularization


\begin{figure}[t]
% \setlength{\abovecaptionskip}{6pt}
\centering
\includegraphics[width=0.49\textwidth]{figures/intro3.png} 
\caption{Relationship between prevalent regularization strategies and the objective function during the feature selection phase, where $\alpha$ and $\beta$ symbolize the respective importances assigned to each term.}
\label{fig:reg2}
\end{figure}

\subsection{Interplay Between Regularization and Sparsity} \label{part:Sparsity}
We then focus on the relationship between the regularization and the predefined sparsity $\eta$ of targeted subgraph $\mathcal{G}^\ast$, where $\eta=1-|\mathcal{G}^\ast|/|\mathcal{G}|$. 
% Since regularization is the tradeoff term to keep the balance between two phases (\textit{Proposition 1}), we first explore the shifts of above balance when sparsity is fluctuate.
According to Equation \ref{eq:GEIB}, sparsity variation of $\mathcal{G}^\ast$ only affects the objective of feature selection, \textit{i.e.}, $I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}^\ast\right)-I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}\right)$. Therefore, we aim to derive the relation between $\eta$ and the phase of feature selection in current explanation methods. Concretly:

To calculate the above objective, here we follow \cite{GSAT} and introduce the variational approximation $\Space{P}_\phi (\mathcal{G}\odot \mathbf{M} \,|\, \mathcal{G}^\ast)$ for $\Space{P} (\mathcal{G}\odot \mathbf{M} \,|\, \mathcal{G}^\ast)$ and $\Space{Q}$ for marginal distribution $\Space{P} (\mathcal{G}\odot \mathbf{M})$ simultaneously. Then the lower bound of the objective can be derived as:
\begin{equation}\label{eq:lower_bound_feature_selection}
\begin{aligned}
    & I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}^\ast\right)-I\left(\mathcal{G}\odot \mathbf{M};\mathcal{G}\right) \\
\ge\ & \mathbb{E}_{\mathcal{G}\odot \mathbf{M}, \mathcal{G}^\ast}\left[\log \mathbb{P}_\phi\left( \mathcal{G}\odot \mathbf{M}\mid\mathcal{G}^\ast\right)\right]+H(\mathcal{G}\odot \mathbf{M}) \\
    & - \mathbb{E}_{\mathcal{G}\odot \mathbf{M},\mathcal{G}}\left[\operatorname{KL}\left(\mathbb{P}\left(\mathcal{G}\odot \mathbf{M} \mid \mathcal{G}\right) \| \mathbb{Q}\left(\mathcal{G}\odot \mathbf{M}\right)\right)\right].
\end{aligned}
\end{equation} 


Detailed derivation is shown in Appendix. While $\mathbf{M}$ is inherited from feature attribution, Equation \ref{eq:lower_bound_feature_selection} is in positive relation to its first term, $\mathbb{E}_{\mathcal{G}\odot \mathbf{M}, \mathcal{G}^\ast}\left[\log \mathbb{P}_\phi\left( \mathcal{G}\odot \mathbf{M}\mid\mathcal{G}^\ast\right)\right]$, since the rest of terms are constants. To calculate its first term, the variational distribution $\Space{P}_\phi (\mathcal{G}\odot \mathbf{M} \,|\, \mathcal{G}^\ast)$ is defined as follow: for every two directed node pair $(u, v)$ in $\mathcal{G}^\ast$, we sample the elements of $\mathbf{M}$ by $m_{uv} \sim \text{Bern}(z)$ where $z \in [0,1]$ is a hyperparameter. Borrowing the above $\Space{P}_\phi$, the first term of Equation \ref{eq:lower_bound_feature_selection} is equal to: 
\begin{equation}\label{eq:lower_bound_log}
\begin{aligned}
     &\mathbb{E}_{\mathcal{G}\odot \mathbf{M}, \mathcal{G}^\ast}\left[\log \mathbb{P}_\phi\left( \mathcal{G}\odot \mathbf{M}\mid\mathcal{G}^\ast\right)\right] \\
   = & 
     \sum_{(u,v)\in \Set{E}^\ast} m_{uv}\text{ log }\frac{m_{uv}}{z}+(1-m_{uv})\text{ log }\frac{(1-m_{uv})}{1-z},
\end{aligned}
\end{equation}
where $\Set{E}^\ast$ is the set of edges in $\mathcal{G}^\ast$. Note that Equation \ref{eq:lower_bound_log} has positive relation to the number of terms $|\Set{E}^\ast|$, which is equal to  $(1-\eta)|\mathcal{G}|$, since $\mathbf{M}$ is inherent and the values of every terms are fixed. That is, in the phase of feature selection, the lower bound of the objective is in negative relation to $\eta$. 
% It is worth to mention that Equation \ref{eq:lower_bound_log} is similar with the regularization terms proposed in GSAT \cite{GSAT}. However, it is appropriate for mainly post-hoc explainers while terms proposed in GSAT is tailored for itself solely.


Therefore, for an interpreting task appealing to low sparsity, the magnitude of objective in feature selection is large. Since regularization is the tradeoff scheme between two phases (Proposition \ref{part:Two Phase}), it should be loosened to a favorable direction for feature attribution to keep the balance, and vise versa. We illustrate this process in Figure \ref{fig:spa}. Formally:


\textit{\textbf{Propotion 4.2 (Sparsity-adaptive Regularization) }\label{prop:sparsity}
For a certain interpreting task, let $\Mat{K}_i$ and $\Mat{K}_j$ are the optimal coefficient vector of regularization under the predefined explanatory sparsity $\eta _i$ and $\eta _j$. For all $\eta \in (0,1)$ we have: }
\begin{equation}
    \eta _i \ge \eta _j \Leftrightarrow  \Mat{K}_i \ge \Mat{K}_j
\end{equation}

\noindent According to Proposition \ref{prop:sparsity}, we propose a simple yet effective scheme called \underline{S}parsity-adaptive \underline{R}egularization \underline{S}cheme (SRS)  to enhance the performance of existing explainers. Concretely, SRS first seeks for the optimal coefficients $\Mat{K}_i$ under the certain sparsity $\eta_i$ by grid search, then for other sparsity $\eta_j$, SRS sets $\Mat{K}_j$ according to $\Mat{K}_j=\eta_j / \eta_{i } \, \Mat{K}_i$. 
Detailed implementation  are provided in Section \ref{part:exp_1}.
% Specifically, for a certain interpreting task, we first seek for the optimal regularization coefficient $\rm{K}$ under $\eta = 0.5$ by grid search, then we reduce or enlarge $\rm{K}$ proportionally to the variation of $\eta = 0.5$ in $(0.1, ..., 0.9)$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Stochastic Mechanism \& Regularization

\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{figures/icml2.png}
 \caption{Rationale of sparsity adaptive regularization scheme.}\label{fig:spa}
% \vspace{-10pt}
\end{figure}

\subsection{Regularization \& Stochastic Mechanism}  \label{part:stochastic}
In this part we focus on the relationship between the regularization and the stochastic mechanism. Recent years have witnessed a surge in research that focuses on leveraging the stochastic mechanism to enhance the performance of GNNs explainability \cite{PGEx, Refine,GSAT}. Concretely, the probability of graph $\mathcal{G}$ is first factorized as $P(\mathcal{G})=\Pi_{(i, j) \in \mathcal{E}} P\left(e_{i j}\right)$, where $e_{i j}=1$ if the edge $(i, j)$ exists, and 0 otherwise. Then the Bernoulli distribution is employed to instantiate $P\left(e_{i j}\right)$, where the stochastic mechanism is introduced in this process \cite{PGEx}. Meanwhile, the gumbel-softmax reparameterization trick is applied to make sure the gradient in the Bernoulli distribution is traceable \cite{GUMBOL-SOFTMAX}. However, despite the satisfactory performance of the stochastic mechanism, current researches mainly neglected the theoretical basis of the stochastic mechanism.

We argue that the stochastic mechanism bolsters the explanation methods via facilitating the feature selection. Specifically, employing the stochastic mechanism to the training stage of $\mathbf{M}$ can be regarded as adding random noise to $\mathbf{M}$ \cite{open-black-box}. The entropy of the mask’s distribution will continue to increase during this process under the constraints of the information bottleneck. That in turn maximizes the conditional entropy $H(\mathcal{G} | \mathcal{G} \odot \mathbf{M})$. Since the entropy of input graph $H(\mathcal{G})$ is a constant, mutual information $I(\mathcal{G}\odot \mathbf{M}, \mathcal{G})=H(\mathcal{G})-H(\mathcal{G} | \mathcal{G} \odot \mathbf{M})$ is minimized contributed to stochastic mechanism. In conclusion, the stochastic mechanism can accelerate the process of minimizing $I(\mathcal{G}\odot \mathbf{M}, \mathcal{G})$, thus endowing the compression of the explanatory subgraph. That is, it can be regarded as the implicit regularization term in favor of the phase of feature selection, as shown in Figure \ref{fig:sto}. We summarize this rationale as Proposition \ref{prop:stoch} and verify it in Section \ref{part:exp_2}.

\textit{\textbf{Proposition 4.3 (Rationale of Stochastic Mechanism)}\label{prop:stoch}
The stochastic mechanism in current explainers works as the implicit regularization term, which endows GNNs explainability with better compressibility.}

\begin{figure}[htp]
 \centering
 \includegraphics[width=0.80\linewidth]{figures/icml3.png}
 \caption{Rationale of stochastic mechanism 
in explainability: an implicit regularization term.}\label{fig:sto}
% \vspace{-10pt}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  OOD \& Regularization

\subsection{Regularization \& OOD }\label{part:ood}
Many recent endeavors have been made towards revealing the out-of-distribution issue of the post-hoc explanation methods \cite{fjfnips,fjfwsdm,www22_ood, DIR, GSAT}. Concretely, OOD issue is posed in the data space since the distribution of full graph $\Space{P}(\mathcal{G})$ differs from that of subgraph $\Space{P}(\mathcal{G}_s)$ \textit{w.r.t.} some properties of graph data such as size \cite{sizeood}, degree \cite{degreeood} and homophily \cite{pinyuood}. Thus it is fallacious to leverage the original GNN $f$, which is trained for the full graphs, to estimate the MI in terms of subgraphs. Unfortunately, most previous explainers \cite{GNNEx,PGEx,PGMEx,GSAT} simply feed $\mathcal{G} \odot \mathbf{M}$  into $f$, unaware of that 
$I\left(f(\mathcal{G} \odot \mathbf{M} );\mathbf{Y}\right)$ is not proportional to $I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right)$, sometimes not even close.

To reveal the relationship between OOD issue and regularization, we scrutinize the OOD between $\Space{P}(\mathcal{G})$ and $\Space{P}(\mathcal{G}_s)$ and decouple it into two phases: (1) OOD between $\Space{P}(\mathcal{G})$ and $\Space{P}(\mathcal{G} \odot \mathbf{M})$ posed in feature attribution, termed OOD-AT and (2)  OOD between $\Space{P}(\mathcal{G}\odot \mathbf{M})$ and $\Space{P}(\mathcal{G}_s)$ posed in feature selection,  termed OOD-SE.

\textbf{OOD-AT.} We first focus on OOD-AT posed in feature attribution. 
According to Equation \ref{eq:OOD_attri_all},  feature attribution searches for the optimal $\mathbf{M}$ via calculating the cross-entropy $H(f(\mathcal{G} \odot \mathbf{M}),\mathbf{Y})$ to approximate  $I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right)$. The approximation error - illustrated as \textit{gap1} in Figure \ref{fig:two_phases} - is given as the sum of second and third term of Equation \ref{eq:OOD_attri_all}. The second term, \textit{i.e.,} $H(\mathbf{Y})$  is the constant across candidates $\mathbf{M}$ thus would not affect the result. Unfortunately, for the third term, \textit{i.e.,} $\operatorname{KL}\left(\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right) ||\, \mathbb{P}_\theta\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right)\right)$, OOD-AT makes this part far away from zero and inevitably fluctuate across different $\mathbf{M}$.

% H(\mathbf{Y})
% \\
% &+\mathbb{E}_{\mathcal{G} \odot \mathbf{M} }\left[\operatorname{KL}\left(\mathbb{P}\left(\mathbf{Y} \,|\, \mathcal{G} \odot \mathbf{M} \right) ||\, \mathbb{P}_\theta\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right)\right)

% As described in Section \ref{part:Two Phase},  feature attribution approximates $I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right)$ by estimating the cross-entropy $H(f(\mathcal{G} \odot \mathbf{M} \,|\, \Theta),\mathbf{Y})$. The error of approximation can be derived from Equation (\ref{eq:OOD_attri_all}):
% \begin{equation}
% I\left(\mathcal{G} \odot \mathbf{M} ; \mathbf{Y}\right)-H(f(\mathcal{G} \odot \mathbf{M} \,|\, \Theta),\mathbf{Y}) \ge \mathbb{E}_{\mathcal{G} \odot \mathbf{M}}\left[\operatorname{KL}\left(\mathbb{P}\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right) \| \mathbb{P}_\theta\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right)\right)\right]. \label{eq:OOD_at}
% \end{equation}
% Note that $\Space{P}_\theta$ depends on distribution $\Space{P}(\mathcal{G})$ since its instantiation  $f(\cdot\,|\, \Theta)$ is trained for $\mathcal{G}$; and $\Space{P}$ depends on the distribution $\Space{P}(\mathcal{G} \odot \mathbf{M})$ since $\mathbf{Y}$ is given. Thus, distribution shift between $\Space{P}(\mathcal{G})$ and $\Space{P}(\mathcal{G}\odot \mathbf{M}$) leads to the fluctuation of above approximation error across different candidates $\mathbf{M}$. 
This fluctuation degrades the fairness of the searching process of optimal $\mathbf{M}$, and further degenerates the effectiveness of the mapping, $\mathcal{G} \mapsto \mathcal{G} \odot \mathbf{M}$ in feature attribution. 
% Thus we formulate the tangible impact caused by OOD-AT as:
% \begin{equation}\label{eq:OOD_at_propotional}
% \begin{aligned}
% \text{OOD}\propto\mathbb{D}_{\mathbf{M}}[\operatorname{KL}\left(\mathbb{P}\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right) \| \mathbb{P}_\theta\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right)\right)], 
% \end{aligned}
% \end{equation}
Thus the tangible impact caused by OOD-AT is proportional to: $\mathbb{D}_{\mathbf{M}}[\operatorname{KL}\left(\mathbb{P}\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right) \| \mathbb{P}_\theta\left(\mathbf{Y} \mid \mathcal{G} \odot \mathbf{M} \right)\right)]$,
where $\mathbb{D}$ is the \textit{Variance}. If regularization pushes $\Space{P}(\mathcal{G} \odot \mathbf{M})$ close to $\Space{P}(\mathcal{G})$ via constraining $\mathbf{M}$ to $\mathbf{A}$, this \textit{Variance} would close to zero and OOD-AT will cause little degradation. Note that this process is similar to the left side of Figure \ref{fig:two_phases}: the constrain orientation is loosened to $\mathbf{A}$ to eliminate the gap.

% According to Equation (\ref{eq:OOD_at_propotional}), if we adjust regularization scheme to push $\mathbf{M}$ to $\mathbf{A}$, $\mathcal{G} \odot \mathbf{M}$ will be close to OOD-AT and $\text{OOD}_\text{at}$ will cause little degradation. 


\textbf{OOD-SE.} We then focus on OOD-SE posed in feature selection. While feature selection binarizes  $\mathbf{M}$ to get $\mathbf{M}'$ and generates $\mathcal{G}_s=\mathcal{G} \odot \mathbf{M}'$, the degree of OOD-SE can be simplified as the distance between $\mathbf{M}$ and $\mathbf{A}_s$. That is, OOD-SE issue will be remedied if regularization pushes $\Space{P}(\mathcal{G} \odot \mathbf{M})$ close to $\Space{P}(\mathcal{G}_s)$ via constraining $\mathbf{M}$ to $\mathbf{A}_s$.


In conclusion, just similar to the dilemma of regularization between two phases described in Section \ref{part:Two Phase}, the optimal regularization scheme for remedying OOD-AT and OOD-SE is totally different. That is, there is inherent uncooperativeness between OOD in feature attribution and selection. Note that above analysis also explains why OOD issue is the inherent limitation of post-hoc explainability: since we can only remedy one side and ignore the other side, OOD can not be thoroughly settled by adjusting the training objective and hyperparameters solely. In a nutshell:

\textit{\textbf{Proposition 4.4 (Rationale of OOD)}\label{prop:ood}
    The OOD issue is imputed to the contradictory effects of regularization on the phases of feature attribution and selection.}

Even though the OOD issue is inherent, we introduce a simple yet effective regularization scheme called \underline{O}OD-resistant \underline{R}egularization \underline{S}cheme (ORS) to alleviate the above dilemma to some extent. Specifically, in the early stage of training, loose regularization of $\mathbf{M}$ is performed in favor of alleviating OOD-AT for the more precise mapping $\mathcal{G} \mapsto \mathcal{G}\odot\mathbf{M}$. Similarly, we then gradually tighten the regularization of $\mathbf{M}$ to alleviate the OOD-SE for the mapping $\mathcal{G}\odot\mathbf{M}\mapsto\mathcal{G}^\ast$. ORS can achieve better explanation performance than the common invariable regularization scheme.  Detailed implementation is provided in Section \ref{part:exp_2}.
